MeshUDF: Fast and Differentiable Meshing of Unsigned Distance Field Networks

Unsigned Distance Fields (UDFs) can be used to represent non-watertight surfaces. However, current approaches to converting them into explicit meshes tend to either be expensive or to degrade the accuracy. Here, we extend the marching cube algorithm to handle UDFs, both fast and accurately. Moreover, our approach to surface extraction is differentiable, which is key to using pretrained UDF networks to fit sparse data.

==> figs/CHD_MC_res.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	 \includegraphics[clip, trim={0cm 0 0.8cm 0},width=.47\textwidth]{figs/CHD_MC_res_p.pdf}
%    \vspace{-20pt}
	\end{center}
		 \caption{\textbf{Chamfer distance at varying grid resolutions:} between reconstructed meshes and ground truth shapes, for two meshing procedures, averaged over the 300 training garments of MGN. Our method yields constantly accurate meshes. By contrast, \textit{Inflation} significantly deforms shapes at low resolutions.}
	\label{fig:CHD_MC_res}
	% \vspace{-10pt}
\end{figure}


==> figs/artefact.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	\begin{overpic}[width=.48\textwidth]{figs/artefact_p.pdf}

		\put(15,-2){\small{(a)}}
		\put(68,-2){\small{(b)}}

	\end{overpic}

%   \vspace{-10pt}
	\end{center}
		 \caption{\textbf{Removing artifacts}: \textbf{(a)}
		 With the $0$-surface in blue, red cells have gradients in opposing directions and yield undesirable surface elements. We prune these by evaluating the UDF on reconstructed triangles.
		 \textbf{(b)} Initially reconstructed borders are uneven (top insert). We smooth them in a post-processing step (bottom).}
	\label{fig:artefact}
	% \vspace{-12pt}
\end{figure}


==> figs/choice_eps.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	\begin{overpic}[width=.45\textwidth]{figs/choice_eps_p.pdf}
		\put(6,27){\small{$s$}}
		\put(13.5,22.6){\small{\color{red}{$2\epsilon$}}}
		\put(64.7,22.6){\small{\color{red}{$2\epsilon$}}}
	\end{overpic}

%    \vspace{-20pt}
	\end{center}
		 \caption{\textbf{Choice of $\epsilon$ for \textit{Inflation}}: when meshing a UDF field's $\epsilon$'s iso-level with standard marching cubes, the chosen value of $\epsilon$ is lower bounded by half the step size $s$. \textbf{Left}: $2\epsilon<s$ produces many large holes. \textbf{Right}: $2\epsilon \geq s$ produces a watertight mesh.}
	\label{fig:choice_eps}
	% \vspace{-10pt}
\end{figure}


==> figs/method_AND_artefact.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\begin{figure}[t]
	\centering
	%%% Left: method
	\begin{minipage}{.485\textwidth}
		\centering
		% \vspace{8pt}
		\begin{overpic}[width=\textwidth]{figs/method_p.pdf}
			\put(8.5,20){\small{$u_1$}}
			\put(2,18.5){\small{$\bgrad_1$}}
			\put(21.5,20){\small{$u_2$}}
			\put(28.5,20.5){\small{$\bgrad_2$}}
			\put(21.5,5.5){\small{$u_3$}}
			\put(28.5,7){\small{$\bgrad_3$}}
			\put(8.5,5.5){\small{$u_4$}}
			\put(1,5){\small{$\bgrad_4$}}
			% Signed distances
			\put(42,25.5){\small{$s_1 \text{=} u_1$}}
			\put(44,20.){\small{$s_2 \text{=-} u_2$}}
			\put(44,.1){\small{$s_3 \text{=-} u_3$}}
			\put(42,5.5){\small{$s_4 \text{=} u_4$}}
			% Linear interpolation
			\put(78.2,18.5){\small{$\tfrac{s_1}{s_1-s_2}$}}
			% a, b, c
			\put(15,-7.5){\small{(a)}}
			\put(49,-7.5){\small{(b)}}
			\put(83,-7.5){\small{(c)}}
		\end{overpic}
		% \vspace{-1pt}
		\captionof{figure}{\textbf{Detecting surface crossings}: \textbf{(a)} all corners of the cell are annotated with unsigned distance values $u_i$ and gradients $\bgrad_i$ ; \textbf{(b)} we locally approximate signed distances with $s_i {=} \text{sgn}(\bgrad_1 \cdot \bgrad_i) u_i$ ; \textbf{(c)} marching cubes processes these pseudo-signed distances and produces a surface element accordingly.}
		\label{fig:method}
	\end{minipage}%
	% \hspace{2mm}
	\begin{minipage}{.485\textwidth} %%% Right: artefact cause and removal
		\centering
		\begin{overpic}[width=\textwidth]{figs/artefact_p.pdf}
			\put(15,0){\small{(a)}}
			\put(68,0){\small{(b)}}
		\end{overpic}
		% \vspace{-17pt}
		\captionof{figure}{\textbf{Removing artifacts}: \textbf{(a)} With the blue $0$-level, the red cell has gradients in opposing directions and yields an undesirable face. We prune these by evaluating the UDF on reconstructed faces. \textbf{(b)} Initially reconstructed borders are uneven (top), we smooth them in post-processing (bottom).}
		\label{fig:artefact}
	\end{minipage}
	% \vspace{-7mm}
\end{figure}


==> figs/method_diff.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	\begin{overpic}[width=.48\textwidth]{figs/method_diff_p.pdf}
		\put(15.5,27){\small{$\bn$}}
		\put(20.3,8){\small{$\bv_-$}}
		\put(20,14.5){\small{$\bv$}}
		\put(19.8,20.4){\small{$\bv_+$}}
		\put(45.5,11.5){\footnotesize{$\alpha$}}

		\put(0.5,6){\textcolor{darkgray}{\scriptsize$\text{=}0$}}
		\put(1,14){\textcolor{darkgray}{\scriptsize$>\!\!0$}}
		\put(0.5,0){\textcolor{darkgray}{\scriptsize$>\!\!0$}}

		\put(22.5,-2){\small{(a)}}
		\put(72.5,-2){\small{(b)}}

		\put(71,17){\small{$\bv'$}}
		\put(71,11){\textcolor{gray}{\small{$\bv$}}}

	\end{overpic}

%   \vspace{-10pt}
	\end{center}
		 \caption{\textbf{Iso-surface deformation}: \textbf{(a)} with $\bv$ on the $0$-levelset, we surround it with $\bv_+$ and $\bv_-$ at a distance $\alpha$ ; \textbf{(b)} In case the UDF decreases at $\bv_+$ and increases at $\bv_-$, $\bv$ moves to $\bv'$.}
	\label{fig:method_diff}
\end{figure}


==> figs/method_diff_border.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	\begin{overpic}[clip, trim={0cm 0.8cm 0 0.1cm},width=.48\textwidth]{figs/method_diff_border_p.pdf}

		\put(28,7){\small{$\bv$}}
		\put(34,7){\small{$\bv_o$}}
		\put(41,2.5){\small{$\bo$}}
		\put(32.5,0.5){\footnotesize{$\alpha$}}
		\put(75,7){\small{$\bv'$}}
		\put(87,7){\textcolor{gray}{\small{$\bv$}}}

		\put(3.5,0){\textcolor{darkgray}{\tiny$\text{=}0$}}
		\put(3,7){\textcolor{darkgray}{\tiny$>\!\!0$}}

		\put(22.5,-2){\small{(a)}}
		\put(72.5,-2){\small{(b)}}

	\end{overpic}

%   \vspace{-10pt}
	\end{center}
		 \caption{\textbf{Iso-surface shrinkage/extension}: \textbf{(a)} with $\bv$ on the border of the $0$-levelset, we place $\bv_o$ at a distance $\alpha$ in the direction of $\bo$ ; \textbf{(b)} If the UDF increases at $\bv_o$, $\bv$ moves to $\bv'$.}
	\label{fig:method_diff_border}
	% \vspace{-7pt}
\end{figure}


==> figs/ndf_chibane.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	 \includegraphics[width=.45\textwidth]{figs/ndf_chibane_p.pdf}
%    \vspace{-20pt}
	\end{center}
		 \caption{\textbf{Applying our method to NDF~\cite{Chibane20b}}, a point cloud completion network.
	\label{fig:ndf_chibane}
\end{figure}


==> figs/optim_PC.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US

\setlength{\tabcolsep}{3pt}
\begin{figure}[t]
	\begin{center}
	\begin{tabular}{cccc}
	 \includegraphics[width=.1\textwidth]{figs/fit_PC/gt.png}&
	 \includegraphics[width=.1\textwidth]{figs/fit_PC/CHD.png} &
	 \includegraphics[width=.1\textwidth]{figs/fit_PC/surf.png} &
	 \includegraphics[width=.1\textwidth]{figs/fit_PC/surf_vol.png} \\
			(a) & (b) & (c) & (d)
	\end{tabular}
	\end{center}
	% \vspace{-7mm}
		\caption{\textbf{Optimizing from sparse point clouds:} \textbf{(a)} Ground truth mesh sparsely sampled, \textbf{(b)} Reconstruction when fitting $\mathbf{z}$ with $\mathcal{L}_{PC,mesh}$ using our differentiable meshing procedure, \textbf{(c)} when using $\mathcal{L}_{PC,UDF}$ in the UDF domain, \textbf{(d)} similarly with $\widetilde{\mathcal{L}}_{PC,UDF}$.}
	\label{fig:optim_PC}
	% \vspace{-10pt}
\end{figure}
\setlength{\tabcolsep}{6pt}


==> figs/optim_silh.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\setlength{\tabcolsep}{3pt}
\begin{figure}
	\begin{center}
	\begin{overpic}[width=.47\textwidth]{figs/optim_silh_p.pdf}

		\put(16,1){\small{(a)}}
		\put(49,1){\small{(b)}}
		\put(82,1){\small{(c)}}

	\end{overpic}
	\end{center}
	% \vspace{-7mm}
		 \caption{\small \textbf{Fitting to binary silhouettes.} \textbf{(a)} Superposition of the target silhouette (light gray) and latent vector initialization (dark gray) \textbf{(b)} After optimizing with differentiable rendering, allowed by our method ($\mathcal{L}_{silh,mesh}$) or \textbf{(c)} with SMPLicit~\cite{Corona21} ($\mathcal{L}_{silh,UDF}$).}
	\label{fig:optim_silh}
	% \vspace{-10pt}
\end{figure}
\setlength{\tabcolsep}{6pt}


==> figs/results.tex <==
% !TEX root = ../eccv2022submission.tex
% !TEX spellcheck = en-US


\begin{figure}
	\begin{center}
	 \includegraphics[width=.47\textwidth]{figs/results_p.pdf}
%    \vspace{-17pt}
	\end{center}
		 \caption{\textbf{Comparison of UDF meshing methods:} Left to right: NDF, Inflation, Ours. Note the inflation at the sleeve's extremity.}
	\label{fig:results}
	% \vspace{-13pt}
\end{figure}

